FeMLoc: Federated Meta-learning for Adaptive Wireless Indoor Localization Tasks in IoT Networks

The rapid growth of the Internet of Things fosters collaboration among connected devices for tasks like indoor localization. However, existing indoor localization solutions struggle with dynamic and harsh conditions, requiring extensive data collection and environment-specific calibration. These factors impede cooperation, scalability, and the utilization of prior research efforts. To address these challenges, we propose FeMLoc, a federated meta-learning framework for localization. FeMLoc operates in two stages: (i) collaborative meta-training where a global meta-model is created by training on diverse localization datasets from edge devices. (ii) Rapid adaptation for new environments, where the pre-trained global meta-model initializes the localization model, requiring only minimal fine-tuning with a small amount of new data. In this paper, we provide a detailed technical overview of FeMLoc, highlighting its unique approach to privacy-preserving meta-learning in the context of indoor localization. Our performance evaluation demonstrates the superiority of FeMLoc over state-of-the-art methods, enabling swift adaptation to new indoor environments with reduced calibration effort. Specifically, FeMLoc achieves up to 80.95% improvement in localization accuracy compared to the conventional baseline neural network (NN) approach after only 100 gradient steps. Alternatively, for a target accuracy of around 5m, FeMLoc achieves the same level of accuracy up to 82.21% faster than the baseline NN approach. This translates to FeMLoc requiring fewer training iterations, thereby significantly reducing fingerprint data collection and calibration efforts. Moreover, FeMLoc exhibits enhanced scalability, making it well-suited for location-aware massive connectivity driven by emerging wireless communication technologies.

==> common/biography.tex <==
\vspace{11pt}

\bf{If you include a photo:}\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}

\vspace{11pt}

\bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiographynophoto}{John Doe}
Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
\end{IEEEbiographynophoto}

\vfill

==> sections/draft.tex <==
\section{ML Model selection}


The aim of this model is to develop an fl framework that learns to select the best suitable ML algorithm given new localization task, by:

\begin{itemize}
    \item Local selecting best optimizer for a given model
    \item Selecting best ML model, autoML
    \item In general, model configurations
\end{itemize}

\subsection{Motivation}
When dealing with positioning task, it hard to know in advance which model will perform the best in a specific environment, and how it has to be optimized.

Personalization of federated model: "Federated learning would need to train a large n-way classifier to utilize data from all clients, while a k-way classifier suffices since it makes predictions for one client each time"

Reducing the number of participationg dvice to reduce training cost. Train a federated meta leraner of client's model initialization

The FL predicts output for the same set of client used in the training, inability to handle a new/unsen client.

implicit data augmentation, improved transfer learning

\textit{Indoor positioning relies on relative positions. The localization is tight to the geometry of the indoor wireless infrstructure making difficult the transferability. Seamless indoor positioning}

\subsection{The federating training}
Collaborative meta-model construction. Collaboration among IoT devices
Synchronous/ asynchronous participation in the training.

Different sources of datasets, each defining a task.
A task can be defined by: an FL device, local dataset, set of usable models, and loss function.

what to communicate to the server at each FL round? Data relevant features, model (CNN, MLP, ...) metadata, reported performance. 

The input to the metafedloc? meta-features of the dataset
Output: a recommendation for the potentially best performing algorithm(s) and its hyper-parameters to solve that task ---Rephrase

Challenge for unseen datasets: use  a similarity measure between data metafeatures and the datbase ones to match the results. 


\subsection{Challenge}
\begin{itemize}
    \item Number of local SGD steps, hyperparameters, ... for each device
    \item trade-off computation vs. communication cost

    \item Asynchronous learning: whenever a device has finished the local training , uploads.
    \item theoritical convergence speed
    \item Joint optimal RIS placement for enhanced positioning using meta learning. Using RIS to create virtual Tx to enhance the meta learning.
    
\end{itemize}

\section{Next directions}
\subsubsection{Test best}
A design of a test bed intended to assess the metalloc practical experiment.

\begin{definition}[Federated meta-learning problem]
  \begin{itemize}
  https://arxiv.org/pdf/2110.14216v2.pdf/ definition fl problem
      \item Set of possible data, parameter space, each data element associated with an element in parameter space.
      \item collection of clients, each associated with a dataset
      \item distribution on client, then the global learning function.
  \end{itemize}
\end{definition}

\begin{remark}[Client selection]
  remark
\end{remark}

\begin{definition}[Dimensionality change loss]
  loss
\end{definition}

\begin{definition}[Information loss - reduction]
  loss
\end{definition}
\begin{definition}[Information gain - augmentation]
  gain
\end{definition}

\begin{definition}[Generalization error bound]
  The minimum error of the meta-model on new unseen data without fine-tuning.
\end{definition}

In FeMLoc, what we refer to  by iteration coincides with the communication round in FL and with episode in meta-learning terminology.
Our work set apart from SoA by: (i) L, (ii) L, and (iii) L

\section{Contribution}
\begin{itemize}
    \item Model compatibility:
    \item Network interoperability
    \item Fast adaptation
    \item Collaborative framework: foster collaboration among iot deviced
    \item Communication efficiency 
\end{itemize}

why con3D ? The num\_BS is used to eumlate the RGB channel in immage processing. In the indoor enviromnment, since the csi capture at different bs may have spatial correlation, we use a 3D kernel for the convolution, hence the 3D. (To be proven by comparing the implementation of conv2d and con3d)

Whenever ther's a change in the envoronme,nt, like change in antennas orientations, offline APs, new APs deploiment, environm,et designchqges, the aim is to quickly fine tune the existingg model to meet the new requirments, eliminqting to need to repeat the localizatiion system design.

The number of input channels of the CNN can be regarded as the number of available access points. The CNN will then then generate a latent CSI image with a consensus output channels set a the standard number of capture APs of the meta model.

\section{Back to RSSI}
Besides, since RSSI is the most sigbal characteristic used for localization, we give a second look at it and show that our model can be adaopted with rssi measurement. We measure the trannsferability of this meta meta model to RSSI locxalization task through OTDD mesure.

Clustering:

\section{Vs. meta learning}
- In FmL, the client model is updated at each iteration, as in FL
- in Meta just at initialization
- The FmL model is update like in meta not like in FL

FmL dos this:
- The global model is trained model in the meta learning way
- The client are trained in the FL way
\section{Problem}
``Furthermore, the existing approaches train and evaluate the models for
specific environments and tasks separately. Moreover, the transferability and adaptability of the
pre-trained fully-supervised representations of the existing models are unknown. To address these
fundamental concerns, we propose a''

\section{Continual learning facilitate by FeMLoc}
With femloc, a good initialization is provided and continues the learning as new task are added along the way.

\section{Inclusion of RSSI Databases survey}
\begin{table}[]
\begin{tabular}{llllllll}
Reference    & signal type & Publication date & building & floor & Area   & \#Recording & \#WAPs \\
UJIIndoorLoc \cite{ujiindoorloc} & Wi-Fi      & 2014    & 3        & 13    & 108703 & 21048(1997 + 1111)    & 520 \\
TUT2017  \cite{lohan_elena_simona_2017_889798} & Wi-Fi   & 2017  & 1 & 5  &2,570(208x108)& 4648(697+3951)   & 991  \\
TUT2018 \cite{philipp_richter_2018_1161525}    & Wi-Fi     & 2018      & 1     &  3  &    --    & 1428 (446+982) & 489 \\
IEEEDataport \cite{49yg-5d21-19} & Wi-Fi & 2019 & 1 & 2 & 24,000 & 7175 & 72\\
UJILIBDB \cite{ltmsupport} & Wi-Fi &2017 & 1& 2& -- &63,504 & 448\\
% MSIData \cite{} &Wi-Fi \& BLE & 2022 & 1 & 3 &386.25 & --& 42+17\\
HDLCDataset \cite{hybrid} &Wi-Fi \& BLE & 2022 & 1 & 3 &386.25 & & 42+17 \\
UTSIndoorLoc \cite{utsindoorloc} &  Wi-Fi &2019 & 1& 16 & 44,000 &  9494 (9107 + 387 ) &  589  \\
UTMInDualSymFi \cite{utm} & Wi-Fi& 2022& 4& 14& & 53300& 250\\
DSIData \cite{dsi} & Wi-Fi& 2020& 1& 1& -- &1717 & 157\\
MSIData \cite{msi} & Wi-Fi& 2019 & 1& 1& 1000 & 28915& 11\\
MTUT\_SAH1 \cite{mtut} & Wi-Fi &2021 & 1& 3& --& 9447& 775 \\
MTUT\_TIE1 \cite{mtut} & Wi-Fi &2021 & 1& 6 & -- &10683 & 613\\
IEEEDataport \cite{} & & & & & & & \\
IEEEDataport \cite{} & & & & & & & \\ 
\end{tabular}
\end{table}
\section{Meta learning with these data}
Goal: >=15 indoor loc databases




Federated meta-learning is an advanced and innovative approach that combines the principles of federated learning and meta-learning to address challenges related to dynamic and distributed data environments. It builds upon the strengths of both paradigms to create a powerful framework capable of adapting and learning efficiently across a network of decentralized clients while rapidly adapting to new tasks and environments.

1. **Federated Learning**:
   Federated learning is a decentralized machine learning approach where multiple clients collaboratively train a shared model without sharing raw data (McMahan et al., 2017). Instead of centralizing data on a single server, model updates occur locally on individual clients, and only aggregated model updates are shared. Federated learning ensures data privacy and minimizes communication costs, making it suitable for scenarios with sensitive data or limited network resources.

2. **Meta-Learning**:
   Meta-learning, or "learning to learn," focuses on training models that can quickly adapt to new tasks with limited data (Finn et al., 2017). Meta-learning involves two phases: meta-training and fine-tuning. In the meta-training phase, models are exposed to a variety of tasks, learning a set of initial parameters that enable rapid adaptation. During fine-tuning, these initial parameters are adjusted using a small amount of task-specific data.

3. **Federated Meta-Learning**:
   Federated meta-learning extends the concept of meta-learning to a federated setting. In this approach, multiple clients each possessing their own task-specific data sources participate in the meta-learning process. The framework involves two levels of learning: the global level and the local level.

   - **Global Level**: At the global level, a central server coordinates the meta-training process. It aggregates model updates from individual clients, creating a shared global model. This model captures high-level knowledge across all tasks and clients in the federated network.

   - **Local Level**: At the local level, each client utilizes its local data to adapt the global model to its specific task or environment. Local updates, inspired by meta-learning principles, enable rapid task-specific adaptation using minimal data.

4. **Advantages of Federated Meta-Learning**:
   - **Data Privacy**: Federated meta-learning maintains data privacy by performing model updates locally on client devices, ensuring that sensitive data remains on-premises.
   - **Scalability**: The federated approach is inherently scalable, enabling collaboration across a large number of clients and tasks without the need for centralized data storage.
   - **Adaptability**: The combination of federated learning and meta-learning provides a flexible and adaptive framework that can quickly adapt to changes in data distribution, tasks, and environments.
   - **Generalization**: Federated meta-learning enhances the generalization capabilities of models by leveraging knowledge from multiple clients and tasks, improving overall model performance.
   - **Efficiency**: By leveraging both federated learning's communication efficiency and meta-learning's data-efficient adaptation, federated meta-learning offers a powerful solution for distributed and dynamic learning scenarios.

Federated meta-learning has promising applications in various domains, including healthcare, finance, and Internet of Things (IoT), where data is distributed across multiple devices or locations. It holds the potential to revolutionize collaborative machine learning by enabling efficient and adaptable learning across diverse and evolving data sources.
